Deployment of High Energy Physics software with a standard method

The installation and maintenance of scientific software for research in experimental, phenomenological, and theoretical High Energy Physics (HEP) requires a considerable amount of time and expertise. While many tools are available to make the task of installation and maintenance much easier, many of these tools require maintenance on their own, have little documentation and very few are used outside of HEP community. For the installation and maintenance of the software, we rely on the well tested, extensively documented, and reliable stack of software management tools with the RPM Package Manager (RPM) at its core. The precompiled HEP software packages can be deployed easily and without detailed Linux system knowledge and are kept up-to-date through the regular system update process. The precompiled packages were tested on multiple installations of openSUSE, RHEL clones, and Fedora. As the RPM infrastructure is adopted by many Linux distributions, the approach can be used on more systems. In this contribution, we discuss our approach to software deployment in detail, present the software repositories for multiple RPM-based Linux distributions to a wider public and call for a collaboration for all the interested parties.

==> Makefile <==
#ulimit -u 10000
latexfile?=HR
newname?=HR
STYLE=proceedings


LATEX=  lualatex -halt-on-error -shell-escape -enable-write18
LATEX=  pdflatex -halt-on-error -shell-escape -enable-write18
BIBTEX=bibtex
UNAME_S := $(shell uname -s)
ifeq ($(UNAME_S),Linux)
SED=sed
endif
ifeq ($(UNAME_S),Darwin)
SED=gsed
endif



latexfiles=  $(latexfile)-txt.tex $(latexfile)-val.tex 
ifeq ($(STYLE),proceedings)
	latexfiles=
	STYLE_SPECIFIC_FILES=$(latexfile)-proceedings.tex jpconf.cls jpconf11.clo TheP8I.spec gitlab-ci.xml HR.bib iopart-num.bst
endif


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex $(latexfile).bst
endif

ifeq ($(STYLE),arxiv)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-arxiv.tex $(latexfile).bst
endif

ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex $(latexfile).bst
endif


all: $(latexfile)-$(STYLE).pdf

tar:  Makefile $(figures) $(constanttables) $(tables)   $(latexfiles) $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	cp Makefile   $(latexfiles)  $(latexfile).bib   $(STYLE_SPECIFIC_FILES) TAR
ifeq ($(STYLE),epjc)
	cp $(figures) TAR/
else
	#mkdir -p TAR/Figures
	#cp $(figures) TAR/Figures
endif
	$(SED) -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	$(SED) -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	$(SED) -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	$(SED) -i '/@artic/achecked={2},'     TAR/*bib	
	$(SED) -i '/@inproceed/achecked={2},' TAR/*bib	
	$(SED) -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	$(SED) -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	$(SED) -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	$(SED) -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	$(SED) -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif

ifneq ($(STYLE),proceedings)
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
endif
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
ifeq ($(STYLE),epjc)
	$(SED) -i 's@Figures/@@g' TAR/Makefile
endif
ifeq ($(STYLE),proceedings)
	#mv TAR/$(latexfile)-def.tex TAR/$(newname)-def.tex
	#cat TAR/$(latexfile)-val.tex | grep [:0-9:] > TAR/$(newname)-val.tex
	#rm -f  TAR/$(newname)-txt.tex TAR/$(latexfile).bst TAR/$(newname).bst 
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
	#rm -rf TAR/$(newname).bib 
endif
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),epjc)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
	tar -zcvf   $(newname).tar.gz -C TAR . 
	rm -rf $(newname).zip; cd TAR; zip ../$(newname).zip ./*/* ./*; cd ..

	rm -rf TAR


figures=  
tables=
constanttables=


$(latexfile)-$(STYLE).pdf :  $(figures) $(constanttables) $(tables) \
                    $(latexfiles)  $(latexfile).bib  $(STYLE_SPECIFIC_FILES) 
                    #answers.tex
	#$(LATEX) answers.tex
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	$(SED) -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	$(SED) -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	$(SED) -i 's@Collaboration@Coll\.@g'  $(latexfile)-$(STYLE).bbl
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)

pdf : $(latexfile)-$(STYLE).pdf

$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
	for a in $$(ls -1 $(latexfile)-*.tex ); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t --dont-tex-check-comments -d en_GB -c $$a ;\
	done

clean :
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm


